Joint Representation Learning and Novel Category Discovery on Single- and Multi-modal Data

This paper studies the problem of novel category discovery on single- and multi-modal data with labels from different but relevant categories. We present a generic, end-to-end framework to jointly learn a reliable representation and assign clusters to unlabelled data. To avoid over-fitting the learnt embedding to labelled data, we take inspiration from self-supervised representation learning by noise-contrastive estimation and extend it to jointly handle labelled and unlabelled data. In particular, we propose using category discrimination on labelled data and cross-modal discrimination on multi-modal data to augment instance discrimination used in conventional contrastive learning approaches. We further employ Winner-Take-All (WTA) hashing algorithm on the shared representation space to generate pairwise pseudo labels for unlabelled data to better predict cluster assignments. We thoroughly evaluate our framework on large-scale multi-modal video benchmarks Kinetics-400 and VGG-Sound, and image benchmarks CIFAR10, CIFAR100 and ImageNet, obtaining state-of-the-art results.

==> wat_alg.tex <==
\begin{algorithm}[t]
\caption{WTA hash}\label{alg:wta}
\begin{algorithmic}[1]
\State \textbf{Preparation:}
\State Extract feature vector by $x = f_\theta(I)$.
\State Generate permutation set $\mathcal{P} = \{\rho_1, ..., \rho_m\}$, set window size $\omega$.
\State \textbf{Main loop:}
\For{$\rho_i \in \mathcal{P}$}
  \State Permute $x$ by $x'=\rho_i(x)$.  
  \State $top_{k}\left(\rho_i\left(x_i)\right)\right)$.
\EndFor
\State \textbf{Obtain optimal:}
\State Let $K^*_a$ be the value of $K$ that maximise ACC for $D^l_{rv}$ and $K^*_v$ be the value that maximise CVI for $D^u$ and let $\hat K = (K^*_a + K^*_v)/2$. Run semi-supervised $K$-means on $D^l_r \cup D^u$ again assuming $L_r+\hat K$ classes.
\State \textbf{Remove outliers:}
\State Look at the resulting clusters in $D^u$ and drop any that has a mass less than $\tau$ of the largest cluster. Output the number of remaining clusters.
\end{algorithmic}
\end{algorithm}
